Unconstrained Road Marking Recognition with Generative Adversarial Networks

Recent road marking recognition has achieved great success in the past few years along with the rapid development of deep learning. Although considerable advances have been made, they are often over-dependent on unrepresentative datasets and constrained conditions. In this paper, to overcome these drawbacks, we propose an alternative method that achieves higher accuracy and generates high-quality samples as data augmentation. With the following two major contributions: 1) The proposed deblurring network can successfully recover a clean road marking from a blurred one by adopting generative adversarial networks (GAN). 2) The proposed data augmentation method, based on mutual information, can preserve and learn semantic context from the given dataset. We construct and train a class-conditional GAN to increase the size of training set, which makes it suitable to recognize target. The experimental results have shown that our proposed framework generates deblurred clean samples from blurry ones, and outperforms other methods even with unconstrained road marking datasets.

==> name.tex <==





\bibitem{c1} Wu, Tao, and Ananth Ranganathan. "A practical system for road marking detection and recognition." Intelligent Vehicles Symposium (IV), 2012 IEEE. IEEE, 2012.
\bibitem{c2} Ahmad, Touqeer, et al. "Symbolic road marking recognition using convolutional neural networks." Intelligent Vehicles Symposium (IV), 2017 IEEE. IEEE, 2017.
\bibitem{c3} Goodfellow, Ian, et al. "Generative adversarial nets." Advances in neural information processing systems. 2014.
\bibitem{c4} Redmon, Joseph, and Ali Farhadi. "YOLO9000: better, faster, stronger." arXiv preprint (2017).
\bibitem{c5} Burrow, M. P. N., H. T. Evdorides, and M. S. Snaith. "Segmentation algorithms for road marking digital image analysis." Proceedings of the Institution of Civil Engineers-Transport. Vol. 156. No. 1. Thomas Telford Ltd, 2003.
\bibitem{c6} Li, Hua, Mingyue Feng, and Xiao Wang. "Inverse perspective mapping based urban road markings detection." Cloud Computing and Intelligent Systems (CCIS), 2012 IEEE 2nd International Conference on. Vol. 3. IEEE, 2012.
\bibitem{c7} Greenhalgh, Jack, and Majid Mirmehdi. "Automatic detection and recognition of symbols and text on the road surface." International Conference on Pattern Recognition Applications and Methods. Springer, Cham, 2015.
\bibitem{c8} Rosten, Edward, Reid Porter, and Tom Drummond. "Faster and better: A machine learning approach to corner detection." IEEE transactions on pattern analysis and machine intelligence 32.1 (2010): 105-119.
\bibitem{c9} Dalal, Navneet, and Bill Triggs. "Histograms of oriented gradients for human detection." Computer Vision and Pattern Recognition, 2005. CVPR 2005. IEEE Computer Society Conference on. Vol. 1. IEEE, 2005.
\bibitem{c10} Matas, Jiri, et al. "Robust wide-baseline stereo from maximally stable extremal regions." Image and vision computing 22.10 (2004): 761-767.
\bibitem{c11} Kheyrollahi, Alireza, and Toby P. Breckon. "Automatic real-time road marking recognition using a feature driven approach." Machine Vision and Applications 23.1 (2012): 123-133.
\bibitem{c12} Krizhevsky, Alex, Ilya Sutskever, and Geoffrey E. Hinton. "Imagenet classification with deep convolutional neural networks." Advances in neural information processing systems. 2012.
\bibitem{c13} Simonyan, Karen, and Andrew Zisserman. "Very deep convolutional networks for large-scale image recognition." arXiv preprint arXiv:1409.1556 (2014).
\bibitem{c14} Radford, Alec, Luke Metz, and Soumith Chintala. "Unsupervised representation learning with deep convolutional generative adversarial networks." arXiv preprint arXiv:1511.06434 (2015).
\bibitem{c15} Chen, X., Duan, Y., Houthooft, R., Schulman, J., Sutskever, I., & Abbeel, P. (2016). Infogan: Interpretable representation learning by information maximizing generative adversarial nets. In Advances in neural information processing systems (pp. 2172-2180).
\bibitem{c16} Sabokrou, M., M. Fathy, and M. Hoseini. "Video anomaly detection and localisation based on the sparsity and reconstruction error of auto-encoder." Electronics Letters 52.13 (2016): 1122-1124.
\bibitem{c17} Bailo, Oleksandr, et al. "Robust road marking detection and recognition using density-based grouping and machine learning techniques." Applications of Computer Vision (WACV), 2017 IEEE Winter Conference on. IEEE, 2017.
\bibitem{c18} Lin, Tsung-Yi, et al. "Microsoft coco: Common objects in context." European conference on computer vision. Springer, Cham, 2014.
\bibitem{c19} Kingma, Diederik P., and Jimmy Ba. "Adam: A method for stochastic optimization." arXiv preprint arXiv:1412.6980 (2014).
\bibitem{c20} Ioffe, Sergey, and Christian Szegedy. "Batch normalization: Accelerating deep network training by reducing internal covariate shift." arXiv preprint arXiv:1502.03167 (2015).
\bibitem{c21} Ledig, Christian, et al. "Photo-realistic single image super-resolution using a generative adversarial network." arXiv preprint (2017).
\bibitem{c22} Bai, Yancheng, et al. "Finding tiny faces in the wild with generative adversarial network." CVPR. IEEE (2018).
\bibitem{c23} Radford, Alec, Luke Metz, and Soumith Chintala. "Unsupervised representation learning with deep convolutional generative adversarial networks." arXiv preprint arXiv:1511.06434 (2015).
\bibitem{c24} Gulrajani, Ishaan, et al. "Improved training of wasserstein gans." Advances in Neural Information Processing Systems. 2017.
